Beyond the Frame: Single and mutilple video summarization method with user-defined length

Video smmarization is a crucial method to reduce the time of videos which reduces the spent time to watch/review a long video. This apporach has became more important as the amount of publisehed video is increasing everyday. A single or multiple videos can be summarized into a relatively short video using various of techniques from multimodal audio-visual techniques, to natural language processing approaches. Audiovisual techniques may be used to recognize significant visual events and pick the most important parts, while NLP techniques can be used to evaluate the audio transcript and extract the main sentences (timestamps) and corresponding video frames from the original video. Another approach is to use the best of both domain. Meaning that we can use audio-visual cues as well as video transcript to extract and summarize the video. In this paper, we combine a variety of NLP techniques (extractive and contect-based summarizers) with video processing techniques to convert a long video into a single relatively short video. We design this toll in a way that user can specify the relative length of the summarized video. We have also explored ways of summarizing and concatenating multiple videos into a single short video which will help having most important concepts from the same subject in a single short video. Out approach shows that video summarizing is a difficult but significant work, with substantial potential for further research and development, and it is possible thanks to the development of NLP models.

==> 3-Experiments.tex <==
\section{Experimental Setup}










Figure \ref{fig:OverallMethodology} depicts the methodology of video summarization using abstractive text summarization. The process starts with data collection, where data is extracted from YouTube videos using the YouTube API. Then, the extracted text is preprocessed to remove stop words, punctuations and perform other necessary transformations.
The preprocessed text is then fed into an abstractive text summarizer that generates a summary of the video content. The summarizer employs NLP techniques such as semantic analysis and language modeling to produce a high-quality summary that captures the essence of the video.
Next, frames are selected that correspond to the summary generated by the text summarizer. The frames are selected based on their relevance to the summary, and the objective is to choose frames that can effectively convey the key points of the video.
The selected frames are then concatenated to form a video summary. The concatenation process involves stitching together the selected frames in a meaningful way, such that the resulting video provides a concise and informative representation of the original video content.
Finally, the output video summary is produced, which can be used as a standalone representation of the original video or as an aid to navigate through the video content.

\subsection{Data collection}
The process of converting audio to text is a crucial step in many applications, including speech recognition, natural language processing, and data analysis. In recent years, advancements in machine learning and artificial intelligence have led to significant improvements in the accuracy and efficiency of audio-to-text conversion systems.

The first step in our methodology is to collect video data from YouTube using the YouTube API. This involves specifying the search query parameters to retrieve videos related to our topic of interest. From each video, we will extract the video ID and use it to obtain the corresponding video transcript.
The next step in the process is to convert the audio from the video into text format using automatic speech recognition (ASR) technology. ASR technology uses machine learning algorithms to convert spoken words into text, making it possible to analyze and process the content of the video.
One of the most popular ASR models is Google Cloud Speech-to-Text, which is capable of accurately transcribing audio in over 120 languages and dialects. The model uses deep neural networks to analyze audio signals and convert them into text, making it highly accurate and capable of handling noisy and complex audio inputs.
Another commonly used ASR model is Amazon Transcribe, which uses advanced machine learning algorithms to transcribe audio in real-time. The model is capable of handling multiple audio formats, including streaming audio, making it ideal for use in real-time applications such as live broadcasts or conference calls.
In addition to cloud-based ASR models, there are also open-source ASR models such as Mozilla DeepSpeech and Kaldi, which can be trained on custom datasets and customized to meet specific requirements. These models offer greater flexibility and control over the transcription process, but may require more technical expertise to set up and use.
After the audio has been converted to text, the resulting transcript can be further processed to remove irrelevant information such as background noise, filler words, and other extraneous details. This preprocessing step helps to ensure that the resulting text is as accurate and relevant as possible, which is essential for downstream analysis and applications.



\subsection{Text preprocessing}
Preprocessing the transcripts is a crucial step to ensure that the resulting summary is concise and relevant. To achieve this, we will employ various techniques to remove irrelevant information, such as stop words, punctuation marks, and timestamps. Stop words are common words that are often removed from text to improve the efficiency of information retrieval. These include words such as "the", "and", "is", and "in". Punctuation marks, such as commas and periods, also do not carry significant meaning in text and can be safely removed. Additionally, timestamps are not relevant for the summarization task and can be removed as well.
There are various existing models and techniques that can be used for text preprocessing, including the Natural Language Toolkit (NLTK) in Python, the Stanford CoreNLP library, and the spaCy library. NLTK provides a comprehensive suite of libraries and tools for natural language processing tasks, such as tokenization, stemming, and stop word removal. Stanford CoreNLP is a Java-based library that provides a range of natural language processing tools, including sentence splitting, tokenization, and named entity recognition. spaCy is another popular Python library for natural language processing, which includes features such as part-of-speech tagging, dependency parsing, and entity recognition. These tools can help automate the text preprocessing task and ensure that the resulting summary is both accurate and concise.

\subsection{Abstractive summarization}
Abstractive text summarization is a challenging natural language processing task that involves understanding the meaning of a given text and generating a concise summary in natural language that captures the key points of the original content. Unlike extractive summarization, which involves selecting and combining sentences from the original text, abstractive summarization aims to create a summary that is not restricted to the exact wording of the original text. Instead, it generates a new summary that is grammatically correct and semantically meaningful, while preserving the important information from the original text.

To achieve this, we will use an abstractive text summarizer, which is a type of neural network model that can learn to generate natural language summaries from a given text input. Specifically, we will train a sequence-to-sequence neural network model with attention on a large corpus of summaries and their corresponding transcripts. This type of model has shown promising results in recent years for a variety of natural language processing tasks, including text summarization.
There are several existing models and techniques that can be used for abstractive text summarization, including the Transformer model and its variants, such as BERT and GPT-3. The Transformer model, which was introduced in 2017, has significantly improved the performance of abstractive summarization tasks, as it can learn to attend to different parts of the input text when generating the summary. BERT and GPT-3 are even more advanced models that have been pre-trained on large amounts of text data and can be fine-tuned for specific natural language processing tasks, including text summarization.
Other models and techniques for abstractive text summarization include the Pointer-Generator network, which can generate both extractive and abstractive summaries, and the Hierarchical Attention Network, which can summarize long documents by hierarchically aggregating information from different levels of the document. These models and techniques can provide valuable insights and tools for abstractive text summarization, and can help improve the accuracy and efficiency of the summarization process.

\subsection{Video processing}
Computer vision techniques play a crucial role in the video summarization process by enabling the identification of key frames that correspond to the summary. This involves analyzing the visual content of the video and identifying the frames that best represent the key concepts and ideas presented in the summary.
One popular computer vision technique for video summarization is keyframe extraction, which involves selecting a set of frames from the video that best represent the content of the video as a whole. This can be done manually by a human expert, or using automated techniques such as clustering, histogram analysis, or machine learning algorithms. Once the keyframes have been identified, they can be concatenated to create a summary video that provides a concise and visually appealing overview of the original video content.
Another approach for video summarization is to use object detection and recognition techniques to identify specific objects or events in the video that are relevant to the summary. This can be done using deep learning models such as YOLO, Faster R-CNN, or Mask R-CNN, which can detect and track objects in real-time video streams. By focusing on the objects or events that are most relevant to the summary, this approach can provide a more focused and informative summary video.
Other computer vision techniques that can be used for video summarization include scene segmentation, which involves dividing the video into segments based on changes in the visual content, and optical flow analysis, which can detect and track motion in the video. These techniques can provide additional information about the visual content of the video and help identify key frames that are most relevant to the summary.



